Blind Channel Equalization Using Vector-Quantized Variational Autoencoders

State-of-the-art high-spectral-efficiency communication systems employ high-order modulation formats coupled with high symbol rates to accommodate the ever-growing demand for data rate-hungry applications. However, such systems are more vulnerable to linear and nonlinear transmission impairments, and it is important to mitigate the performance loss via digital signal processing. In this paper, we propose a novel machine learning approach for blind channel equalization and estimation using the vector quantized (VQ) \ac{VAE} framework. The proposed approach generalizes the applicability of the conventional \ac{VAE}-based equalizer to nonlinear systems employing high-order modulation formats by introducing a codebook component and an associated novel loss function. We evaluate the performance of the proposed method over a linear additive white Gaussian noise channel with intersymbol interference and two nonlinear scenarios. Simulation results show that the proposed method can achieve similar performance as a data aided equalizer using the \acf{MMSE} criterion, and outperforms the blind\ac{CMA} and the \ac{VAE}-based channel equalizer. Furthermore, we show that for the linear channel, the proposed scheme exhibits better convergence properties than the \ac{MMSE}-based, the \ac{CMA}-based, and the \ac{VAE}-based equalizers in terms of both convergence speed and robustness to variations in training batch size and learning rate.

==> VQ-VAE-based-Channel-Equalization (Arxiv)/Acronym.tex <==
\DeclareAcronym{AE}{
short=AE,
long= autoencoder,
}

\DeclareAcronym{WDM}{
short=WDM,
long=wavelength division multiplexing ,
}

\DeclareAcronym{NN}{
short=NN,
long= neural network,
}
\DeclareAcronym{DSP}{
short=DSP,
long= digital signal processing,
}
\DeclareAcronym{CMA}{
short=CMA,
long= constant modulus algorithm,
}

\DeclareAcronym{MMA}{
short=MMA,
long= multi-modulus algorithm,
}


\DeclareAcronym{PS}{
short= PS,
long= pulse-shaping,
}


\DeclareAcronym{DAC}{
short=DAC,
long= digital-to-analog converter,
}

\DeclareAcronym{ADC}{
short=ADC,
long= analog-to-digital converter,
}



\DeclareAcronym{DL}{
short=DL,
long= direct learning,
}

\DeclareAcronym{ENOB}{
short=ENOB,
long= effective number of bits,
}

\DeclareAcronym{DPD}{
short= DPD,
long= digital pre-distortion,
}


\DeclareAcronym{}{
short=,
long= ,
}

\DeclareAcronym{MZM}{
short= MZM,
long= Mach-Zehnder modulator ,
}

\DeclareAcronym{MZI}{
short= MZM,
long= Mach-Zehnder interferometer ,
}
\DeclareAcronym{ML}{
short= ML,
long= maximum-likelihood  ,
}
\DeclareAcronym{VAE}{
short= VAE,
long= variational autoencoder  ,
}

\DeclareAcronym{VQ-VAE}{
short= VQ-VAE,
long= vector quantized VAE  ,
}


\DeclareAcronym{EDFA}{
short= EDFA,
long= erbium-doped fiber amplifier ,
}

\DeclareAcronym{SE}{
short= SE,
long= spectral efficiency ,
}

\DeclareAcronym{PA}{
short= PA,
long= power amplifier ,
}

\DeclareAcronym{MF}{
short= MF,
long= matched filter ,
} 

\DeclareAcronym{OOB}{
short= OOB,
long= out-of-band ,
}

\DeclareAcronym{ICI}{
short= ICI,
long= inter-channel interference,
}

\DeclareAcronym{IQM}{
short= IQM,
long= in-phase and quadrature modulator,
}



\DeclareAcronym{RRC}{
short= RRC,
long= root-raised-cosine,
}

\DeclareAcronym{AWGN}{
short= AWGN,
long= additive white Gaussian noise,
}

\DeclareAcronym{SER}{
short= SER,
long= symbol error rate,
}
\DeclareAcronym{BER}{
short= BER,
long= bit error rate,
}

\DeclareAcronym{RL}{
short= RL,
long= reinforcement learning,
}

\DeclareAcronym{SNDR}{
short= SNDR,
long= signal-to-noise-plus-distortion ratio,
}

\DeclareAcronym{SNR}{
short= SNR,
long= signal-to-noise ratio,
}

\DeclareAcronym{FIR}{
short= FIR,
long= finite impulse response,
}

\DeclareAcronym{KL}{
short= KL,
long=Kullback-Leibler,
}

\DeclareAcronym{VI}{
short= VarInf,
long=variational inference,
}

\DeclareAcronym{MC}{
short= MC,
long=Monte-Carlo,
}

\DeclareAcronym{pmf}{
short= pmf,
long=conditional probability mass function,
}

\DeclareAcronym{LE}{
short= LE,
long=linear equalizer,
}

\DeclareAcronym{MMSE}{
short= MMSE,
long=minimum-mean-squared-error,
}

\DeclareAcronym{MSE}{
short= MSE,
long= mean squared error,
}
 
 \DeclareAcronym{FFE}{
short= FFE,
long=feed-forward equalizer,
}

\DeclareAcronym{ELBO}{
short= ELBO,
long= evidence lower bound,
}
 
 
 
\DeclareAcronym{SSMF}{
short= SSMF,
long= standard single mode fiber,
}


\DeclareAcronym{NZDSF}{
short= NZDSF,
long=non-zero dispersion-shifted fiber,
}


\DeclareAcronym{ISI}{
short= ISI,
long= inter-symbol interference,
}

\DeclareAcronym{GMP}{
short= GMP,
long= generalized memory polynomial,
}

\DeclareAcronym{MP}{
short= MP,
long= memory polynomial,
}


\DeclareAcronym{PDF}{
short= PDF,
long= probability density function,
}

\DeclareAcronym{MAP}{
short= MAP,
long=  maximum a posterior,
}

\DeclareAcronym{iid}{
short= i.i.d.,
long=  independent and identically distributed,
}


\DeclareAcronym{DBP}{
short= DBP,
long=  digital backpropagation}



\DeclareAcronym{FEC}{
short= FEC,
long=  forward error correction}





\DeclareAcronym{SPS}{
short= SPS,
long=  samples per symbol}


 
 \DeclareAcronym{SL}{
short= SL,
long= supervised learning}



\DeclareAcronym{DD-LMS}{
short= DD-LMS,
long=  decision-directed least-mean-squares}




==> VQ-VAE-based-Channel-Equalization (Arxiv)/figures/common.tex <==
\usepackage[tbtags]{amsmath}
\usepackage{nccmath}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{bm}
\usepackage{color}
\usepackage{verbatim}
\usepackage{balance}
\usepackage{graphicx}
% \usepackage[font={footnotesize}]{caption}
% \captionsetup[figure]{font=small,skip=0pt}
% \setlength{\abovecaptionskip}{-15pt}

% \usepackage{array, ltablex, multirow,ragged2e}
\usepackage{booktabs,siunitx, multirow,ragged2e}
\usepackage{hyperref}
% \usepackage{longtable}
% \usepackage{mdframed}


% \usepackage{subfig} 
\usepackage{dsfont}
\usepackage{cite}
\usepackage{float}
\usepackage{algorithm}
\usepackage[noend]{algpseudocode}
%\usepackage{tikz,pgfplots,tkz-graph}
\usepackage{tikz,pgfplots}
\usepgfplotslibrary{fillbetween}
\usepgfplotslibrary{groupplots}
\makeatletter
\def\BState{\State\hskip-\ALG@thistlm}
\makeatother
\usepackage{xcolor}



\graphicspath{{../figures/}}
\pgfplotsset{compat=newest}%
\usetikzlibrary{positioning,matrix,shapes.multipart,shapes.misc,spy}%
\interdisplaylinepenalty=2500%
\tikzstyle{annotation}=[fill=white]%
\usepackage{balance}
\usepackage{acro}

\usepackage{xcolor}



\definecolor{VAE_color}{rgb}{0, 1, 0.3}
\definecolor{CMA_color}{rgb}{0,0,0}

\definecolor{MMSE_color}{rgb}{0, 0, 1}

\definecolor{VQ_VAE_color1}{rgb}{1, 0, 0} %%% red
\definecolor{VQ_VAE_color2}{rgb}{1, 0.2, 0.2}
\definecolor{VQ_VAE_color3}{rgb}{1, 0.5, 0.3}

\definecolor{VQ_VAE_color4}{rgb}{1, 0.3, 0.6}



\newcommand{\vect}[1]{\bm{#1}}
\newcommand{\mat}[1]{\bm{#1}}
\newcommand{\transpose}{\top}
\newcommand{\Ctranspose}{\dagger}
\newcommand{\figwidth}{7.3cm}
\newcommand{\figheight}{4.8cm}
% \newcommand{\todo}{\textcolor{red}{#1}}
\newcommand{\todo}[1]{{\color{red}{Todo: #1}}}

\usetikzlibrary{shapes.arrows}
\usetikzlibrary{spy}


\tikzset{%
	partial ellipse/.style args={#1:#2:#3}{%
		insert path={+ (#1:#3) arc (#1:#2:#3)}%
	}%
}%

